Probing Chemical Language Models: Effects of Pre-training and Fine-tuning

Chemical language models (CLMs) are trained with linearized representations such as SMILES, yet it remains unclear which chemically meaningful substructures they encode. To foster a better understanding of CLMs, we conduct a systematic study and probe for 78 molecular substructures across eight pre-trained and six randomly initialized models. We furthermore study how fine-tuning on chemical downstream tasks affects the learned representations of molecular substructures. Our results show that pre-training generally improves molecular structure awareness of CLMs, particularly in the upper layers. Moreover, randomly initialized models already encode ring structures well in the first layer. Our analysis on two chemical downstream tasks further reveals that, interestingly, fine-tuning affects task-relevant molecular substructures more than others, indicating that the changes in the representations follow chemical theory.

==> images/heatmaps/00_heatmap_example.tex <==


\definecolor{darkblue}{rgb}{0, 0, 0.5}
\hypersetup{colorlinks=true,citecolor=darkblue, linkcolor=darkblue, urlcolor=darkblue}


\begin{tikzpicture}[scale=1.3]
  \foreach \y [count=\n] in {
      {0,15,30,10},
      {15,0,40,70},
      {30,40,0,10},
      {10,70,10,0},
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=ablue!\x!jgreen, minimum size=13mm, text=white] at (\m,-\n) {};
      }
    }

  \foreach \y [count=\n] in {
      {-,3.5e-11,5.5e-5,6.7e-13},
      {3.5e-11,-,0.006,0.562},
      {5.5e-5,0.006,-,9.3e-04},
      {6.7e-13,0.562,9.3e-04,-},
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=none, minimum size=8mm, text=white] at (\m,-\n) {\x};
      }
    }
  % column labels
  \foreach \a [count=\i] in {\texttt{GPT-4},\texttt{MIP},\texttt{SEL},\texttt{SIZE}} {
    \node[minimum size=6mm] at (\i,0) {\a};
  }
  % row labels
  \foreach \a [count=\i] in {\texttt{GPT-4},\texttt{MIP},\texttt{SEL},\texttt{SIZE}} {
    \node[minimum size=6mm] at (0,-\i) {\a};
  } 
  \node[shading = axis, shading angle = 90, top color=ablue, bottom color=jgreen, middle color=ablue!70!jgreen, minimum width=3mm, minimum height=50mm, rectangle] at (4.7,-2.5) {};
  
  \node[fill=none, minimum size=3mm, text=black] at (5.1,-4.4) {0.0};
  \node[fill=none, minimum size=3mm, text=black] at (5.1,-0.5) {1.0};

\end{tikzpicture}


\begin{comment}

\definecolor{darkblue}{rgb}{0, 0, 0.5}
\hypersetup{colorlinks=true,citecolor=darkblue, linkcolor=darkblue, urlcolor=darkblue}


\begin{tikzpicture}[scale=1.3]
  \foreach \y [count=\n] in {
      {0,15,30,10},
      {15,0,40,70},
      {30,40,0,10},
      {10,70,10,0},
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=ablue!\x!jgreen, minimum size=13mm, text=white] at (\m,-\n) {};
      }
    }

  \foreach \y [count=\n] in {
      {-,3.5e-11,5.5e-5,6.7e-13},
      {3.5e-11,-,0.006,0.562},
      {5.5e-5,0.006,-,9.3e-04},
      {6.7e-13,0.562,9.3e-04,-},
    } {
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=none, minimum size=8mm, text=white] at (\m,-\n) {\x};
      }
    }
  % column labels
  \foreach \a [count=\i] in {\texttt{GPT-4},\texttt{MIP},\texttt{SEL},\texttt{SIZE}} {
    \node[minimum size=6mm] at (\i,0) {\a};
  }
  % row labels
  \foreach \a [count=\i] in {\texttt{GPT-4},\texttt{MIP},\texttt{SEL},\texttt{SIZE}} {
    \node[minimum size=6mm] at (0,-\i) {\a};
  } 
  \node[shading = axis, shading angle = 90, top color=ablue, bottom color=jgreen, middle color=ablue!70!jgreen, minimum width=3mm, minimum height=50mm, rectangle] at (4.7,-2.5) {};
  
  \node[fill=none, minimum size=3mm, text=black] at (5.1,-4.4) {0.0};
  \node[fill=none, minimum size=3mm, text=black] at (5.1,-0.5) {1.0};

\end{tikzpicture}
\end{comment}

==> tables/fgroup_description.tex <==
\begin{tabular}{ll}
\toprule
Molecular Substructure & Description \\
\midrule
NHOH & NHs or OHs \\
NO & Nitrogens and Oxygens \\
AliphaticCarbocycles & aliphatic (containing at least one non-aromatic bond) carbocycles \\
AliphaticHeterocycles & aliphatic (containing at least one non-aromatic bond) heterocycles \\
AliphaticRings & aliphatic (containing at least one non-aromatic bond) rings \\
AromaticCarbocycles & aromatic carbocycles \\
AromaticHeterocycles & aromatic heterocycles \\
AromaticRings & aromatic rings \\
HAcceptors & Hydrogen Bond Acceptors \\
HDonors & Hydrogen Bond Donors \\
Heteroatoms & Heteroatoms \\
RotatableBonds & Rotatable Bonds \\
SaturatedCarbocycles & saturated carbocycles \\
SaturatedHeterocycles & saturated heterocycles  \\
SaturatedRings & saturated rings  \\
Ring & rings \\
Al\_COO & aliphatic carboxylic acids \\
Al\_OH & aliphatic hydroxyl groups \\
Al\_OH\_noTert & aliphatic hydroxyl groups excluding tert-OH \\
ArN & N functional groups attached to aromatics \\
Ar\_COO & aromatic carboxylic acid \\
Ar\_N & aromatic nitrogens \\
Ar\_NH & aromatic amines \\
Ar\_OH & aromatic hydroxyl groups \\
COO & carboxylic acids \\
COO2 & carboxylic acids \\
C\_O & carbonyl O \\
C\_O\_noCOO & carbonyl O excluding COOH \\
C\_S & thiocarbonyl \\
Imine & Imines \\
NH0 & Tertiary amines \\
NH1 & Secondary amines \\
NH2 & Primary amines \\
N\_O & hydroxylamine groups \\
Ndealkylation1 & XCCNR groups \\
Ndealkylation2 & tert-alicyclic amines (no heteroatoms, not quinine-like bridged N) \\
Nhpyrrole & H-pyrrole nitrogens \\
SH & thiol groups \\
aldehyde & aldehydes \\
alkyl\_halide & alkyl halides \\
allylic\_oxid &  allylic oxidation sites excluding steroid dienone \\
amide & amides \\
amidine & amidine groups \\
aniline & anilines \\
aryl\_methyl & aryl methyl sites for hydroxylation \\
benzene & benzene rings \\
bicyclic & Bicyclic \\
diazo & diazo groups \\
ester & esters \\
ether & ether oxygens (including phenoxy) \\
furan & uran rings \\
guanido & guanidine groups \\
halogen & halogens \\
hdrzine & hydrazine groups \\
hdrzone & hydrazone groups \\
imidazole & imidazole rings \\
imide & imide groups \\
ketone & ketones \\
ketone\_Topliss & ketones excluding diaryl, a,b-unsat. dienones, heteroatom on Calpha \\
lactone & cyclic esters (lactones) \\
methoxy & methoxy groups -OCH3 \\
morpholine & morpholine rings \\
nitrile & nitriles \\
nitro & nitro groups \\
nitro\_arom & nitro benzene ring substituents \\
nitro\_arom\_nonortho & non-ortho nitro benzene ring substituents \\
oxime & oxime groups \\
para\_hydroxylation & para-hydroxylation sites \\
phenol & phenols \\
phenol\_noOrthoHbond & phenolic OH excluding ortho intramolecular Hbond substituents \\
piperdine & piperdine rings \\
piperzine & piperzine rings \\
priamide & primary amides \\
pyridine & pyridine rings \\
sulfide & thioether \\
thiazole & thiazole rings \\
thiophene & thiophene rings \\
unbrch\_alkane & unbranched alkanes of at least 4 members (excludes halogenated alkanes) \\
urea & urea groups \\
\bottomrule
\end{tabular}

==> tables/probing_test_freqs.tex <==
\begin{tabular}{lrrr}
\toprule
Probing task & \multicolumn{3}{c}{\% of molecules w/substructure} \\
\cmidrule(lr){2-4}
 & Seed 42 &  Seed 77 & Seed 4 \\
\midrule
NHOH & 61.20 & 61.51 & 60.86 \\
NO & 95.38 & 95.48 & 95.42 \\
AliphaticCarbocycles & 17.38 & 17.34 & 17.29 \\
AliphaticHeterocycles & 29.50 & 29.54 & 30.05 \\
AliphaticRings & 42.71 & 42.77 & 43.22 \\
AromaticRings & 64.66 & 64.69 & 64.67 \\
AromaticCarbocycles & 49.26 & 48.84 & 49.48 \\
AromaticHeterocycles & 27.84 & 28.32 & 27.61 \\
HAcceptors & 95.94 & 96.14 & 96.03 \\
HDonors & 62.17 & 62.59 & 61.91 \\
Heteroatoms & 97.82 & 97.92 & 97.84 \\
RotatableBonds & 88.03 & 88.13 & 87.86 \\
SaturatedRings & 26.55 & 26.68 & 26.68 \\
SaturatedCarbocycles & 11.27 & 11.21 & 11.04 \\
SaturatedHeterocycles & 17.39 & 17.46 & 17.59 \\
Ring & 85.53 & 85.84 & 86.00 \\
Al\_COO & 7.17 & 7.14 & 7.42 \\
Al\_OH & 21.76 & 21.98 & 21.84 \\
Al\_OH\_noTert & 20.09 & 20.36 & 20.27 \\
ArN & 4.68 & 4.50 & 4.27 \\
Ar\_COO & 2.06 & 2.09 & 2.11 \\
Ar\_N & 23.54 & 23.74 & 22.96 \\
Ar\_NH & 5.59 & 5.83 & 5.48 \\
Ar\_OH & 5.36 & 5.11 & 4.88 \\
COO & 9.20 & 9.19 & 9.48 \\
COO2 & 9.24 & 9.24 & 9.54 \\
C\_O & 42.93 & 43.13 & 43.42 \\
C\_O\_noCOO & 35.73 & 36.13 & 36.20 \\
C\_S & 1.06 & 1.01 & 1.01 \\
Imine & 12.85 & 12.77 & 13.32 \\
ketone & 10.04 & 9.84 & 9.61 \\
NH0 & 57.19 & 57.01 & 57.49 \\
NH1 & 28.09 & 28.98 & 28.75 \\
NH2 & 12.85 & 12.63 & 12.24 \\
N\_O & 1.97 & 1.95 & 2.06 \\
Ndealkylation1 & 3.51 & 3.48 & 3.54 \\
Ndealkylation2 & 3.62 & 3.61 & 3.87 \\
Nhpyrrole & 5.59 & 5.83 & 5.48 \\
SH & 3.23 & 3.26 & 3.12 \\
aldehyde & 2.04 & 2.02 & 2.00 \\
alkyl\_halide & 6.27 & 6.12 & 6.12 \\
allylic\_oxid & 12.45 & 12.53 & 12.56 \\
amide & 14.00 & 14.27 & 14.69 \\
amidine & 5.04 & 5.41 & 5.44 \\
aniline & 13.87 & 13.58 & 13.42 \\
aryl\_methyl & 17.68 & 17.71 & 18.09 \\
benzene & 49.20 & 48.78 & 49.43 \\
bicyclic & 24.58 & 24.25 & 24.30 \\
ester & 10.78 & 11.16 & 11.09 \\
ether & 30.86 & 31.51 & 31.12 \\
furan & 2.37 & 2.66 & 2.63 \\
guanido & 1.56 & 1.64 & 1.59 \\
halogen & 18.18 & 17.68 & 17.57 \\
hdrzine & 2.75 & 2.65 & 2.61 \\
hdrzone & 3.01 & 3.13 & 3.33 \\
imidazole & 3.17 & 3.29 & 3.16 \\
imide & 1.52 & 1.57 & 1.62 \\
ketone\_Topliss & 7.95 & 7.81 & 7.54 \\
lactone & 1.38 & 1.44 & 1.39 \\
methoxy & 10.91 & 11.30 & 11.19 \\
morpholine & 1.12 & 1.18 & 1.14 \\
nitrile & 5.19 & 5.31 & 5.36 \\
nitro & 4.65 & 4.46 & 4.46 \\
nitro\_arom & 2.81 & 2.69 & 2.75 \\
nitro\_arom\_nonortho & 1.77 & 1.71 & 1.71 \\
oxime & 1.71 & 1.76 & 1.74 \\
para\_hydroxylation & 10.64 & 10.49 & 10.81 \\
phenol & 3.87 & 3.75 & 3.58 \\
phenol\_noOrthoHbond & 3.75 & 3.65 & 3.50 \\
piperdine & 3.48 & 3.38 & 3.58 \\
piperzine & 1.17 & 1.23 & 1.21 \\
pyridine & 7.32 & 7.14 & 6.98 \\
priamide & 1.42 & 1.49 & 1.47 \\
sulfide & 6.33 & 6.22 & 6.25 \\
thiazole & 1.45 & 1.55 & 1.46 \\
thiophene & 2.36 & 2.44 & 2.44 \\
unbrch\_alkane & 7.11 & 7.14 & 7.00 \\
urea & 1.76 & 1.70 & 1.71 \\
\bottomrule
\end{tabular}


==> tables/probing_train_sizes.tex <==
\begin{tabular}{lrrr}
\toprule
Probing task& \multicolumn{3}{c}{Train Split Size} \\
\cmidrule(lr){2-4}
 & Seed 42 &  Seed 77 & Seed 4 \\
\midrule
NHOH & 54574 & 54936 & 54628 \\
NO & 5308 & 5374 & 5454 \\
AliphaticCarbocycles & 44174 & 43876 & 44168 \\
AliphaticHeterocycles & 66372 & 66602 & 66996 \\
AliphaticRings & 99440 & 99306 & 99924 \\
AromaticRings & 76818 & 77146 & 77070 \\
AromaticCarbocycles & 75432 & 75536 & 76012 \\
AromaticHeterocycles & 65176 & 64620 & 64144 \\
HAcceptors & 4662 & 4778 & 4826 \\
HDonors & 53418 & 53890 & 53548 \\
Heteroatoms & 2076 & 2060 & 2156 \\
RotatableBonds & 15078 & 15180 & 15118 \\
SaturatedRings & 70664 & 70306 & 71046 \\
SaturatedCarbocycles & 34032 & 33544 & 33866 \\
SaturatedHeterocycles & 42976 & 43060 & 43562 \\
Ring & 23322 & 23484 & 23270 \\
Al\_COO & 14092 & 14152 & 13996 \\
Al\_OH & 52366 & 52306 & 52222 \\
Al\_OH\_noTert & 48914 & 48874 & 48840 \\
ArN & 10872 & 10808 & 11102 \\
Ar\_COO & 3992 & 3956 & 3878 \\
Ar\_N & 56262 & 55878 & 55370 \\
Ar\_NH & 10330 & 10088 & 9820 \\
Ar\_OH & 8548 & 8220 & 8362 \\
COO & 18034 & 18050 & 17816 \\
COO2 & 19182 & 19154 & 18944 \\
C\_O & 68424 & 68080 & 68792 \\
C\_O\_noCOO & 52970 & 52798 & 53526 \\
C\_S & 870 & 812 & 792 \\
Imine & 28506 & 28680 & 28360 \\
ketone & 15014 & 15276 & 15558 \\
NH0 & 75328 & 75390 & 76000 \\
NH1 & 70862 & 70678 & 71058 \\
NH2 & 39752 & 39668 & 40030 \\
N\_O & 3462 & 3568 & 3484 \\
Ndealkylation1 & 14322 & 14354 & 14098 \\
Ndealkylation2 & 13014 & 13062 & 13032 \\
Nhpyrrole & 10330 & 10088 & 9820 \\
SH & 3550 & 3444 & 3436 \\
aldehyde & 4128 & 4054 & 4228 \\
alkyl\_halide & 12224 & 12168 & 12022 \\
allylic\_oxid & 19950 & 20470 & 20198 \\
amide & 19672 & 19528 & 19746 \\
amidine & 9086 & 9024 & 9054 \\
aniline & 27334 & 27340 & 27794 \\
aryl\_methyl & 42070 & 41994 & 41350 \\
benzene & 75432 & 75530 & 76012 \\
bicyclic & 35830 & 35808 & 35426 \\
ester & 15866 & 15856 & 15890 \\
ether & 63050 & 63536 & 63826 \\
furan & 5358 & 5272 & 5252 \\
guanido & 2322 & 2364 & 2346 \\
halogen & 35422 & 35528 & 35384 \\
hdrzine & 3384 & 3348 & 3280 \\
hdrzone & 1754 & 1792 & 1944 \\
imidazole & 7152 & 7336 & 7074 \\
imide & 1254 & 1166 & 1206 \\
ketone\_Topliss & 13072 & 13170 & 13448 \\
lactone & 1930 & 1940 & 2090 \\
methoxy & 22138 & 22602 & 22642 \\
morpholine & 2316 & 2170 & 2256 \\
nitrile & 11304 & 11414 & 11520 \\
nitro & 4444 & 4384 & 4396 \\
nitro\_arom & 2410 & 2418 & 2368 \\
nitro\_arom\_nonortho & 1182 & 1200 & 1116 \\
oxime & 1570 & 1476 & 1556 \\
para\_hydroxylation & 12858 & 12690 & 12736 \\
phenol & 5432 & 5382 & 5422 \\
phenol\_noOrthoHbond & 5354 & 5284 & 5306 \\
piperdine & 10696 & 10720 & 10628 \\
piperzine & 3064 & 3168 & 3176 \\
pyridine & 18140 & 18244 & 18118 \\
priamide & 576 & 556 & 572 \\
sulfide & 9854 & 9744 & 9946 \\
thiazole & 3874 & 3852 & 3782 \\
thiophene & 5610 & 5394 & 5370 \\
unbrch\_alkane & 12118 & 12130 & 11878 \\
urea & 758 & 752 & 768 \\
\bottomrule
\end{tabular}

